Sorting same-size red blood cells in deep deterministic lateral displacement devices

We study deformability-based sorting of same-size RBCs via DLD using an in-house integral equation solver. Our goal is to quantitatively characterize the physical mechanisms that enable the cell separation. To this end, we systematically investigate the effects of the interior fluid viscosity and membrane elasticity of a cell on its behavior. In particular, we consider deep devices in which a cell can show rich dynamics such as taking a particular angular orientation depending on its mechanical property. We have found out that cells moving with a sufficiently high positive inclination angle with respect to the flow direction displace laterally while those with smaller angles travel with the flow streamlines. Thereby, deformability-based cell sorting is possible. The underlying mechanism here is cell migration due to the cell's positive inclination and the shear gradient. The higher the inclination is, the farther the cell can travel laterally. We also assess the efficiency of the technique for dense suspensions. It turns out that most of the cells in dense suspensions does not displace in the lateral direction no matter what their deformability is. As a result, separating cells using a DLD device becomes harder.

==> preambles.tex <==
%\usepackage[sort,compress]{cite} % this doesn't work with elsevier styles
\usepackage{palatino}
\usepackage[usenames]{color}
\usepackage{epsfig}
\usepackage[fleqn,reqno]{amsmath}
\usepackage{amsfonts,amsthm,bm}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{stmaryrd}
%\usepackage{subfigure, appendix}
\usepackage{subfigure}
\usepackage[titletoc]{appendix}
\usepackage{tabularx,booktabs}
\usepackage{graphics,caption}
\usepackage{fancybox}
\usepackage[top=1.2in,bottom=1.2in,left=1in, right=1in]{geometry}
\usepackage{array}
\usepackage{multirow}
\usepackage{wrapfig}
\usepackage{algorithmic,algorithm}
\usepackage{paralist}
\usepackage{ifthen}
\usepackage{enumitem}
\usepackage{tikz,pgfplots,filecontents}
\usepackage{float}
\usepackage{mdframed}
%\usepackage{showkeys}
\usepackage{todonotes}
%\usepackage[disable]{todonotes}

%To see the labels for now.  Will remove later



% Set path for figures
\graphicspath{{./figs/}}

%%%%%%  pdftex  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[pagebackref=false,bookmarks=false]{hyperref} 

\definecolor{dblue}{rgb}{0.03,0.3,0.62}
\definecolor{dorange}{rgb}{1,0.55,0}

\hypersetup{
  bookmarksnumbered=true,
  bookmarksopen=false,
  hypertexnames=false,     
  breaklinks=true,          
  unicode=false,
  pdffitwindow=true,        
  pdfnewwindow=true,        
  colorlinks=true,         
  linkcolor=dblue,
  anchorcolor=red,
  citecolor=dorange,
  filecolor=magenta,
  urlcolor=dblue,
  pdfstartview = FitH,
  %pdftitle = {},
  %pdfsubject = {Subject},
  pdfkeywords = {},
  pdfcreator = {LaTeX with hyperref package}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\renewcommand{\algorithmiccomment}[1]{
%        \settowidth\textLen{\footnotesize\tt// #1}
%        \setlength\resLen{\the\commLen}
%        \addtolength\resLen{-\the\textLen} 
%        \hfill{\footnotesize\tt// #1}\hspace{\the\resLen}}

\definecolor{sblue}{cmyk}{0.98,0.13,0,0.43} % section blue
\definecolor{sblue}{cmyk}{0.98,0.13,0,0.43} % section blue
\newcommand{\csblue} {\color{sblue}}  %\renewcommand{\csblue}{\color{black}}
\newcommand{\cblack} {\color{black}}
\newcommand{\sblue}[1]{{\color{sblue} #1}}

%\newcommand{\todo}[1]{{\color{red}todo: #1}}
\newcommand{\comment}[1]{\sblue{#1}}
\def\gap{\hspace*{.2in}}
\newcommand{\half}[1]{\frac{#1}{2}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\Div}{\mbox{div}\,}
\newcommand{\Grad}{{\nabla}}
\newcommand{\grbf}[1]{\mbox{\boldmath${#1}$\unboldmath}} %\renewcommand{\grbf}[1] {\mathbf{#1}}}
\newcommand{\p}{\partial}
\newcommand{\avg}[1]{\left< #1 \right>}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\algref}[1]{Algorithm~\ref{#1}}
\newcommand{\Lap}{\rotatebox[origin=c]{180}{$\nabla$}}
\newcommand{\Curl}{{\gbf \nabla \times}}

%Bryan's new commands
\newcommand{\xx}{{\mathbf{x}}}
\newcommand{\txx}{{\tilde{\xx}}}
\newcommand{\yy}{{\mathbf{y}}}
\newcommand{\zz}{{\mathbf{z}}}
\newcommand{\ff}{{\mathbf{f}}}
\renewcommand{\SS}{{\mathcal{S}}}
\newcommand{\BB}{{\mathcal{B}}}
\newcommand{\DD}{{\mathcal{D}}}
\newcommand{\EE}{{\mathcal{E}}}
\newcommand{\UU}{{\mathbf{U}}}
\newcommand{\TT}{{\mathcal{T}}}
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\cc}{{\mathbf{c}}}
\newcommand{\uu}{{\mathbf{u}}}
\newcommand{\vv}{{\mathbf{v}}}
\newcommand{\rr}{{\mathbf{r}}}
\newcommand{\nn}{{\mathbf{n}}}
\newcommand{\eeta}{{\boldsymbol\eta}}
\newcommand{\zzeta}{{\boldsymbol\zeta}}
\newcommand{\ttau}{{\boldsymbol\tau}}
\newcommand{\ssigma}{{\boldsymbol\sigma}}
\newcommand{\llambda}{{\boldsymbol\lambda}}

\DeclareMathOperator*{\argmin}{\arg\!\min}
%\renewcommand{\algorithmiccomment}[1]{\hfill \texttt{\% #1}}
\renewcommand{\algorithmiccomment}[1]{\hfill{\footnotesize\tt #1}}


\newcolumntype{C}{>{\centering\arraybackslash} m{2.5cm}}


